Masses and Scaling Relations for Nuclear Star Clusters, and their Coexistence with Central Black Holes

Galactic nuclei typically host either a Nuclear Star Cluster (NSC, prevalent in galaxies with masses $\lesssim 10^{10}M_\odot$) or a Massive Black Hole (MBH, common in galaxies with masses $\gtrsim 10^{12}M_\odot$). In the intermediate mass range, some nuclei host both a NSC and a MBH. In this paper, we explore scaling relations between NSC mass (${\cal M}_{\rm NSC}$) and host galaxy total stellar mass (${\cal M}_{\star,\rm gal}$) using a large sample of NSCs in late- and early-type galaxies, including a number of NSCs harboring a MBH. Such scaling relations reflect the underlying physical mechanisms driving the formation and (co)evolution of these central massive objects. We find $\sim\!1.5\sigma$ significant differences between NSCs in late- and early-type galaxies in the slopes and offsets of the relations $r_{\rm eff,NSC}$--${\cal M}_{\rm NSC}$, $r_{\rm eff, NSC}$--${\cal M}_{\star,\rm gal}$ and ${\cal M}_{\rm NSC}$--${\cal M}_{\star,\rm gal}$, in the sense that $i)$ NSCs in late-types are more compact at fixed ${\cal M}_{\rm NSC}$ and ${\cal M}_{\star,\rm gal}$; and $ii)$ the ${\cal M}_{\rm NSC}$--${\cal M}_{\star,\rm gal}$ relation is shallower for NSCs in late-types than in early-types, similar to the ${\cal M}_{\rm BH}$--${\cal M}_{\star,\rm bulge}$ relation. We discuss these results in the context of the (possibly ongoing) evolution of NSCs, depending on host galaxy type. For NSCs with a MBH, we illustrate the possible influence of a MBH on its host NSC, by considering the ratio between the radius of the MBH sphere of influence and $r_{\rm eff, NSC}$. NSCs harbouring a sufficiently massive black hole are likely to exhibit surface brightness profile deviating from a typical King profile.

==> GB14_Gal_NSC_1Z_short.tex <==
\begin{deluxetable}{p{1.7cm}llllllllll}
\tabletypesize{\footnotesize}
%\rotate % For landscape mode
%\setlength{\tabcolsep}{0.15cm}
\tablecolumns{11}
\tablewidth{0pc} %%% <--- This is important!!! Otherwise it wont compile!!!!
\tablecaption{Photometric masses of Nuclear Star Clusters and their host galaxies. 
%NSC mass is calculated using photometric error weighted 
%average $M/L$s from the \protect\cite{BC03} SSP models for an assumed solar metallicity. NSC host galaxy mass is calculated using \protect\cite{Bell03} 
%$M/L-$colour relations. Details in \S\,\ref{Sect:Data_NSCs}, \ref{Sect:Data_Gal_Mags} and \ref{Sect:HI_Xray_Masses}.  
(Full table available online only)
\label{Table:GB_Gal_NSC}
}
\tablehead{

\colhead{Object} &
\colhead{$m\!-\!M$} &
\colhead{$t$} &
\colhead{\nscsize} &
\colhead{\nscmass} &
\colhead{${\cal M}_{\rm gal,\star}$} &
\colhead{${\cal M}_{\rm gal, HI}$} &
\colhead{NSC} &
\colhead{$M/L_{\rm NSC}$} &
\colhead{Galaxy} &
\colhead{$M/L_{\rm gal}$} \\
\colhead{} &
\colhead{[mag]} &
\colhead{} &
\colhead{[pc]} &
\colhead{[$10^4M_\odot$]} &
\colhead{[$10^7M_\odot$]} &
\colhead{[$10^7M_\odot$]} &
\colhead{filter} &
\colhead{[$M_\odot/L_\odot$]} &
\colhead{filter} &
\colhead{[$M_\odot/L_\odot$]} \\
\colhead{(1)} &
\colhead{(2)} &
\colhead{(3)} &
\colhead{(4)} &
\colhead{(5)} &
\colhead{(6)} &
\colhead{(7)} &
\colhead{(8)} &
\colhead{(9)} &
\colhead{(10)} &
\colhead{(11)}
}
\startdata

DDO078		&27.82     &10. 	   &$3.7_{-0.00}^{+0.1}$&	$19.21_{-0.48}^{+0.48}$&$	1.22_{\pm	0.91    }$&$    0.00_{\pm	0.00    }$&$    VI	$&$	0.92    _{-     0.02    }^{+    0.02    }$&$     B	$&	1.16	\\
ESO138-G10     &30.84	  &7.9  	  &$7.7_{-7.7}^{+0.1}$&		$2427.8_{-60.69}^{+890.19}$&$   1824.23_{\pm    743.8   }$&$    3274.47_{\pm    1432.55 }$&$    I	$&$	0.45    _{-     0.01    }^{+    0.17    }$&$     B	$&	1.16	\\
ESO359-G29     &30.03	  &9.9  	  &$0.5_{-0.5}^{+0.00}$&	$14.84_{-2.39}^{+19.82}$&$      22.48_{\pm      13.03   }$&$    60.82_{\pm      18.2    }$&$    B       $&$	0.7	_{-	0.11	}^{+	0.93	}$&$	 B	$&	1.16	\\
ESO404-G03     &32.58	  &3.9  	  &$2.1_{-0.3}^{+0.1}$&		$121.9_{-36.74}^{+41.07}$&$     2356.09_{\pm    737.05  }$&$    165.51_{\pm     45.73   }$&$    V       $&$	0.63	_{-	0.19	}^{+	0.21	}$&$	 BI	$&	4.48	\\
ESO418-G08     &31.77	  &7.7  	  &$8.3_{-8.3}^{+0.2}$&		$55.11_{-1.38}^{+1.38}$&$       264.05_{\pm     77.07   }$&$    190.96_{\pm     35.18   }$&$    UVI     $&$	0.45	_{-	0.01	}^{+	0.01	}$&$	 BI	$&	1.53	\\
ESO504-G17     &31.84	  &4.1  	  &$2.3_{-1.1}^{+1.7}$&		$124.76_{-3.12}^{+386.77}$&$    232.88_{\pm     188.92  }$&$    255.19_{\pm     82.26   }$&$    U       $&$	0.15	_{-	0.00	}^{+	0.47	}$&$	 BI	$&	1.48	\\
IC0239		&30.76     &6.0 	   &$2.6_{-0.1}^{+0.1}$&	$123.08_{-5.25}^{+6.44}$&$	969.32_{\pm	104.01	}$&$	1516.65_{\pm	453.99	}$&$	BVI	$&$	1.13	_{-	0.05	}^{+	0.06	}$&$	 BV	$&	1.45	\\
IC5332		&29.62     &6.8 	   &$2.2_{-0.2}^{+0.1}$&	$18.00_{-0.45}^{+0.45}$&$	393.26_{\pm	253.18	}$&$	2168.11_{\pm	698.92	}$&$	BI	$&$	0.6	_{-	0.02	}^{+	0.02	}$&$	 B	$&	1.16	\\
NGC1559		&30.91     &5.9 	   &$1.5_{-0.00}^{+0.00}$&	$456.74_{-92.65}^{+69.27}$&$	587.67_{\pm	176.56	}$&$	833.89_{\pm	249.61	}$&$	BVI	$&$	0.99	_{-	0.2	}^{+	0.15	}$&$	 BV	$&	0.53	\\
NGC1569		&27.21     &9.6 	   &$1.00_{-1.00}^{+0.00}$&	$1683.26_{-42.08}^{+42.08}$&$	56.34_{\pm	19.34	}$&$	1242.71_{\pm	658.13	}$&$	UI	$&$	0.6	_{-	0.01	}^{+	0.02	}$&$	 BV	$&	0.37	\\
NGC2903		&29.80     &4.0 	   &$4.3_{-0.00}^{+0.00}$&	$966.52_{-24.16}^{+24.16}$&$	3148.39_{\pm	675.63	}$&$	3057.34_{\pm	492.79	}$&$	VR	$&$	0.45	_{-	0.01	}^{+	0.01	}$&$	 BV	$&	1.47	\\
NGC3344		&31.40     &4.0 	   &$16.5_{-16.5}^{+0.00}$&	$6154.78_{-153.87}^{+153.87}$&$	4032.78_{\pm	692.34	}$&$	2797.51_{\pm	772.98	}$&$	BV	$&$	0.45	_{-	0.01	}^{+	0.01	}$&$	 BV	$&	1.13	\\
NGC4254		&30.97     &5.2 	   &$7.6_{-0.00}^{+0.00}$&	$2916.02_{-72.9}^{+72.9}$&$	2707.32_{\pm	348.59	}$&$	1566.01_{\pm	432.7	}$&$	UV	$&$	1.45	_{-	0.04	}^{+	0.04	}$&$	 BV	$&	1.04	\\
NGC4639		&31.70     &3.5 	   &$10.3_{-0.00}^{+1.5}$&	$1122.41_{-28.06}^{+28.06}$&$	1849.56_{\pm	238.15	}$&$	339.65_{\pm	109.49	}$&$	UB	$&$	0.6	_{-	0.01	}^{+	0.02	}$&$	 BV	$&	1.7	\\
NGC5264		&28.27     &9.7 	   &$0.4_{-0.00}^{+0.00}$&	$58.74_{-1.47}^{+1.47}$&$	34.12_{\pm	4.39	}$&$	172.01_{\pm	43.57	}$&$	VI	$&$	1.18	_{-	0.03	}^{+	0.03	}$&$	 BV	$&	1.11	\\
NGC5300		&31.82     &5.2 	   &$20.6_{-20.6}^{+0.00}$&	$1632.47_{-103.23}^{+46.78}$&$	924.83_{\pm	1480.2	}$&$	295.33_{\pm	61.2	}$&$	BVI	$&$	0.96	_{-	0.06	}^{+	0.03	}$&$	 BI	$&	2.06	\\
NGC5334		&32.78     &5.2 	   &$11.9_{-0.7}^{+0.4}$&	$708.96_{-297.61}^{+174.51}$&$	615.6_{\pm	894.66	}$&$	520.15_{\pm	143.72	}$&$	BVRI	$&$	0.76	_{-	0.32	}^{+	0.19	}$&$	 BI	$&	0.76	\\
NGC5398		&29.60     &7.9 	   &$1.1_{-1.1}^{+0.1}$&	$107.78_{-75.1}^{+16.27}$&$	2636.58_{\pm	2400.82	}$&$	383.26_{\pm	105.9	}$&$	UBVI	$&$	1.45	_{-	1.01	}^{+	0.22	}$&$	 BI	$&	2.96	\\
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\

\enddata

\vspace{-.5cm}
\tablecomments{
Columns: 
(1) NSC host galaxy ID, 
(2) Adopted distance modulus and 
(3) galaxy morphological code \cite[(1-2-3) are the same as in][]{Georgiev&Boeker14}; 
(4) NSC effective radius measured in $F606W$ or $F814W$ or $F450W$ or $F300W$, as available in this order. 
We note that differences in sizes in the different bands are $<10\%$ \protect\cite[see ][for discussion]{Georgiev&Boeker14}; 
(5) NSC mass calculated using the $M/L$ given in (9) for the $F606W$ (V) or $F814W$ (I) or $F450W$ (B) or $F300W$ (U) filter 
in this priority order, e.g. if Colour is $UBVI$, the value is the $M/L_V$ error weighted average from the $M/L_V$s from the 
various colour combinations containing $V$-band. NSC host galaxy stellar and HI mass (6 and 7), where the used colour and 
$M/L_B$ are in (10) and (11).
}

\end{deluxetable}


